Implicit Latent Variable Model for Scene-Consistent Motion Forecasting

In order to plan a safe maneuver an autonomous vehicle must accurately perceive its environment, and understand the interactions among traffic participants. In this paper, we aim to learn scene-consistent motion forecasts of complex urban traffic directly from sensor data. In particular, we propose to characterize the joint distribution over future trajectories via an implicit latent variable model. We model the scene as an interaction graph and employ powerful graph neural networks to learn a distributed latent representation of the scene. Coupled with a deterministic decoder, we obtain trajectory samples that are consistent across traffic participants, achieving state-of-the-art results in motion forecasting and interaction understanding. Last but not least, we demonstrate that our motion forecasts result in safer and more comfortable motion planning.

==> background.tex <==
\section{Background}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.34\textwidth}
        \centering
        \includegraphics[width=.50\textwidth]{images/independent_output_graphical_model.png}
        \caption{Independent output model}
        \label{figure:graphical_models:independent}
    \end{subfigure}
    \begin{subfigure}[t]{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/autoregressive_graphical_model.png}
        \caption{Autoregressive model}
        \label{figure:graphical_models:autoregressive}
    \end{subfigure}
    \begin{subfigure}[t]{.34\textwidth}
        \centering
        \includegraphics[width=.50\textwidth]{images/joint_latent_model.png}
        \caption{Joint latent model}
        \label{figure:graphical_models:joint_latent}
    \end{subfigure}
    \caption{Graphical models of trajectory distribution  
    }
    \label{figure:graphical_models}
\end{figure}


In the context of trajectory prediction, we wish to model the joint distribution $P(Y|X)$ where $Y = \begin{Bmatrix} y_1, y_2, \cdots, y_N \end{Bmatrix}$ represent a set of $N$ interacting actor's future states 
for $T$ timesteps $y_a = \begin{Bmatrix} y_a^1, y_a^2, \cdots, y_a^T \end{Bmatrix}$, and $X= \begin{Bmatrix} x_1, x_2, \cdots, x_N \end{Bmatrix}$ represent the local context around each detected agent coming from a history of LiDAR observations and HD maps. To sidestep the intractability of representing and estimating this distribution, past methods have proposed various factorizations with different levels of conditional independence assumptions: (i) \emph{independent futures} across actors and timesteps \cite{casas2018intentnet, casas2019spatially, chai2019multipath} $p(Y|X) = \prod_a p(y_a | x_a)$ as in Fig.~\ref{figure:graphical_models:independent}, (ii) \emph{autoregressive generation} \cite{rhinehart2018r2p2,2019arXiv190501296R}, as in Fig.~\ref {figure:graphical_models:autoregressive}, which predicts a distribution on the output at a given timestep $y_a^t$ conditioned on the previous timestep output state of all actors, with an optional latent variable $z_a$ per actor \cite{tang2019multiple}:
$$
y_a^t \sim p\left(y_a^t | y_1^{{0:t-1}}, y_2^{{0:t-1}}, \cdots, y_N^{{0:t-1}}, z_a, x_a\right) 
$$
This however, as mentioned before, suffers from the well known problem of cascading/compounding errors \cite{ross2011reduction, lamb_professor_forcing, osa2018algorithmic} \sergio{intuition in our setting}. While scheduled sampling \cite{bengio2015scheduled} has been proposed to mitigate this issue, the objective function underlying this method is improper and leads to an inconsistent learning algorithm \cite{huszar2015not}.











==> model.tex <==
\subsection{Latent Variable Model of Joint Trajectory Distribution}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.34\textwidth}
        \centering
        \includegraphics[width=.50\textwidth]{images/independent_output_graphical_model.png}
        \caption{Independent output model}
        \label{figure:graphical_models:independent}
    \end{subfigure}
    \begin{subfigure}[t]{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/autoregressive_graphical_model.png}
        \caption{Autoregressive model \sergio{Add $z^a$ to generalize it to MFP's formulation}}
        \label{figure:graphical_models:autoregressive}
    \end{subfigure}
    \begin{subfigure}[t]{.34\textwidth}
        \centering
        \includegraphics[width=.50\textwidth]{images/joint_latent_model.png}
        \caption{Joint latent model \\\sergio{needs to be modified to connect every $x_i$ to every $z_j$}}
        \label{figure:graphical_models:joint_latent}
    \end{subfigure}
    \caption{Graphical models of trajectory distribution}
    \label{figure:graphical_models}
\end{figure}

In the context of trajectory prediction, we wish to model the joint distribution $P(Y|X)$ where $Y = \begin{Bmatrix} y^1, y^2, \cdots, y^N \end{Bmatrix}$ represent a set of $N$ interacting actor's future states 
for $T$ timesteps $y^a = \begin{Bmatrix} y^a_1, y^a_2, \cdots, y^a_T \end{Bmatrix}$, and $X= \begin{Bmatrix} x^1, x^2, \cdots, x^N \end{Bmatrix}$ represent the local context around each detected agent coming from a history of LiDAR observations and HD maps. To sidestep the intractability of representing and estimating this distribution, past methods have proposed various factorizations with different levels of conditional independence assumptions: 1) \emph{independent futures} across actors and timesteps $p(Y|X) = \prod_a p(y_a | x_a)$ as in Fig.~\ref{figure:graphical_models:independent}, 2) \emph{autoregressive generation}, as in Fig.~\ref {figure:graphical_models:autoregressive}, which predicts a distribution on the output at a given timestep $y^a_t$ conditioned on the previous timestep state of all actors:
$$
y^a_t \sim p\left(y^a_t | y^1_{{0:t-1}}, y^2_{{0:t-1}}, \cdots, y^N_{{0:t-1}}, x^a\right) 
$$
This however, as mentioned before, suffers from the compounding error problem.

A latent variable formulation factorizes this joint distribution into two components: $P(Y|X) = P(Y|X, Z) P(Z|X)$ as in Fig.~\ref{figure:graphical_models:joint_latent}. Intuitively, we may expect the \emph{encoder} to capture the latent variation due to high level behaviour and interactions (i.e. planned route, yielding to another vehicle), whereas the \emph{decoder} only captures execution uncertainties (i.e. accelerating slightly faster). We make the assumption that, given the latent space, all predictions are conditionally indepdent $P(Y|X, Z) = \prod_{y \in Y} P(y|X, Z)$. This simplification allows us to sample per-actor trajectory distributions independently, with simple parameterized functions. Furthermore, this assumption can be extended to the time dimension which alleviates the compounding error problem that autoregressive models suffer from.

\simon{Still need to figure out how to better call out the key novelty of our method. Ideally, we have some principled way of saying a graph can approximates the joint}
\cole{Agreed on this main point. I think we mention this joint factorization but do not specify that we believe it's novel.}

To leverage the natural geometric and graphical structure of vehicle interactions, we model the scene-level latent space as a set of continuous latent variables $Z = [z^1, z^2, z^3, ..., z^n]$ parameterized by a set of independent gaussians:
$$
Z \sim \mathcal{N}\left(Z | \left[\mu^1, \mu^2, \mu^3, ..., \mu^n \right], \text{diag}\left(\left[\sigma^1, \sigma^2, \sigma^3, ..., \sigma^n \right]\right) \right)
$$
Each partition of the full latent space $Z$ (as shown in Fig.~\ref{figure:graphical_models:joint_latent}) corresponds to a node (i.e. vehicle) in the interaction graph. Here, we emphasize that even though each $z$ implicitly represents an actor in the interaction graph, they are considered a component of the scene-level latent sample. Thus to generate  trajectories with scene-level consistency, it's critical for the decoder $P(y|X,Z)$ to condition on the scene-level latent samples $Z$ instead of only the node-level latent sample $z$ corresponding to the specific actor. This is particularly challenging, since we have a variable number of actors per scene. Fortunately, recent works \cite{alahi2016social, casas2019spatially} have developed network architectures that can deal with this particular challenge.

Similar to standard variational inference approaches, we make the mean-field assumption in modeling the joint distribution over $Z$ to avoid intractability. In other words, samples of each latent variable are conditionally independent given the context $p(Z|X) = \prod_Z p(z|X)$. 

\simon{Might need to clarify what it means to draw a sample from the scene latent variable}
\sergio{Might want to talk about continuous vs. discrete here when we explain the requirements on the decoder}

\iffalse
\simon{background from Cole, integrate more here? or move some back to background? ===========}
In the context of future trajectory prediction, we consider the set of latent variables $\mathbf{Z} = \begin{Bmatrix}\mathbf{z}^1, \mathbf{z}^2, \cdots, \mathbf{z}^N\end{Bmatrix}$ which is conditioned on the local context of a given actor in the scene based on partially observed sensor data $\mathbf{X}$. As the latent variable $\mathbf{z}$ is input to the decoder network, the stochastic function responsible for generating it $p\left(\mathbf{z} \right)$ must learn a partitioning on the space of future trajectories. This space can be discretely sampled as in \cite{tang2019multiple} to capture discrete actions (turning, yielding, etc.) or continuously sampled as in \cite{lee2017desire} to smoothly move between trajectories in the latent space depending on the chosen approximate distribution $q\left(\mathbf{z} | \mathbf{x}\right)$.

The \emph{decoder network} can be implemented as a deterministic function $\mathbf{y}^n = f_\phi\left(\mathbf{z}^{n}\right)$ that maps a latent sample to an actor's future trajectory $\mathbf{y}^n = \begin{Bmatrix} y^n_1, y^n_2, \cdots, y^n_T \end{Bmatrix}$. During inference, multiple latent variables can be sampled for each actor, which are all independent from each other given each individual context. As can be imagined, this will create samples that are not self consistent with each other. In order to get consistent future scenes, it is necessary to model the joint latent of all actors $p\left(\mathbf{z}^1, \mathbf{z}^2, \cdots, \mathbf{z}^N\right)$ which for a given actor can be written as:

$$
p\left(\mathbf{z}^1, \mathbf{z}^2, \cdots, \mathbf{z}^N\right) = 
p\left(\mathbf{z}^1\right)p\left(\mathbf{z}^1 | \mathbf{z}^2, \mathbf{z}^3, \cdots, \mathbf{z}^N \right)
$$

Unfortunately, even for a small number of actors, these probabilities might be intractable to compute. Instead, we can get scene consistent trajectories from independent samples using a modified \emph{decoder network} that can process sampled latent spaces from all actors $f_\phi\left(\mathbf{z}^1, \mathbf{z}^2, \cdots, \mathbf{z}^N\right)$, and network architectures of this type \cite{casas2019spatially, alahi2016social} have been pioneered in recent years.

\simon{background from Cole===========}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/model.pdf}
    \caption{\textbf{Latent SpAGNN} \sergio{Need to replace the gaussians in the drawing by samples (deterministic y given z sample)}}
    \label{fig:model}
\end{figure}

\subsection{Latent SpAGNN}
We propose an extension to Spatially Aware Graphical Neural Networks (SpAGNN) \cite{casas2019spatially}, called Latent SpAGNN, that allows us to model the complex scene-level, multimodal behaviors that urban driving exhibits. In the remainder of this section, we first give an overview of SpAGNN and then explain how we extend this framework to encode the scene into a set of latent variables as well as to decode the latent into a socially-consistent set of trajectories.

\subsubsection{SpAGNN} We follow past works in joint perception and prediction (\cite{luo2018fast, casas2018intentnet, casas2019spatially}) in adopting a two stage pipeline that is trainable end-to-end. Voxelized LiDAR and rasterized high definition maps are first processed by a CNN-based feature extraction backbone, then the shared spatial features are used to inform a detection network that predicts confidence scores and bounding boxes
. In the second stage, we apply Rotated Region of Interest Align (RRoI Align) \cite{ma2018arbitrary} to extract fixed size appearance and context features around each detection in the scene. As in \cite{casas2019spatially}, we further process the per-actor features with a 4-layer CNN with large strides and max-pooling based feature aggregation. 

The SpAGNN (spatially-aware graph neural network) header explicitly models the relationship between actors by iteratively updating the actor states via a message passing process. Fundamentally, the message passing process comes down to a set of operations:
\begin{enumerate}[leftmargin=1em]
    \item \emph{Neighbordhood function}: $U = \mathbf{N}\left(v\right)$ which returns the set of nodes $U$ that are neighbors in the graph to a given node $v$
    \item \emph{Edge function}: $m_{u\rightarrow v} = \mathcal{E}\left(h_u, h_v \right )$ that takes the representation of two nodes and then computes an edge based feature between them.
    \item \emph{Aggregation function}: $a_v = \mathcal{A}\left(\begin{Bmatrix} m_{u\rightarrow v}\end{Bmatrix} : u \in \mathbf{N}\left(v \right ) \right )$ which aggregates the messages for node $v$ from the nodes in it's neighborhood as defined by the above function.
    \item \emph{Update function}: $h_{v}^{'}=\mathcal{U}\left(h_{v}, a_{v}\right)$ which produces a new node representation based on the one prior to the graph propagation and the aggregated message
\end{enumerate}

We follow the edge, aggregation and update functions of SpAGNN \cite{casas2019spatially} which have shown to be effective for modelling the interactions between road users.

\subsubsection{Latent SpAGNN}
\sergio{Not sure start talking about CVAE is the best given that's only the way we train. At the same time, moving that to Learning section would imply moving the posterior head architecture details there, which would also be weird (?)}
We follow the CVAE framework \cite{sohn2015learning} and  extend \cite{casas2019spatially} to consist of 3 components as shown in Fig.~\ref{fig:model}. We parameterize the 3 components as independent headers, but leverage the same per-actor features:
\begin{enumerate}[leftmargin=1em]
    \item \emph{Posterior head} predicts the latents given the scene context and ground truth trajectories $q(Z|X, Y)$ which is only used during training. We use a single layer GRU with input dimension of 2 and hidden state of 64 as the ground truth future encoder shared across all actors. We pass both raw trajectories and encoded trajectories as additional features $\tilde{h}_{posterior} = [h_x, h_y, y]$ to another \cole{another?} SpaGNN header to predict the posterior distribution over latent variables $q(Z|X, Y)$. We parameterize the posterior distribution over each latent node $z$ as independent Gaussians over k-dimension, with some small k \cole{the small k is not very small when you consider that all of the actors make up the $Z$}. In other words,the scene level latent space has $k \times N$ dimensions, where $N$ is the number of actors in the scene.\\  
    \item \emph{Prior head} predicts the latents given scene context $p(Z|X)$. The prior head is similarly parameterized as a SpAGNN header, except that it does not receive the raw or encoded ground truth futures.\\ 
    \item \emph{Decoder head} predicts future trajectories conditioned on a graph of latent variables.

    We augment the per-actor features with the sampled latent variable by direct concatenation: $\tilde{h}_{decoder} = [h_x, z]$ where $h_x$ is the per-actor feature, and $h$ is the node feature as input to the Spatially-Aware Graph Neural Network. Iterative message passing allows the network to explicitly reason about the spatial-temporal relationship between actors, and indirectly condition on the entire scene-level latent $Z=[z^1, z^2, ... z^n]$. As a result, the network is capable of characterizing a joint trajectory distribution that achieves scene-level consistency.
\end{enumerate}

During inference, we draw samples of the latent variable from the prior network $Z \sim p(Z|X)$ and then pass them to the deterministic decoder function to generate a full trajectory for each actor given its individual context.

\cole{Is this what we do? I guess that's what the graph does...}

==> network.tex <==
\subsection{Network Architecture}

\paragraph{Backbone Network}
We combine the ideas in PIXOR \cite{yang2018pixor} and IntentNet \cite{casas2018intentnet} to build a multi-resolution, two-stream backbone network that extracts features from the LiDAR voxelization and map raster, as can be seen in Fig.\ref{fig:diagram}. One stream ($\text{CNN}_\text{L}$) processes LiDAR and the other one ($\text{CNN}_\text{M}$) processes the map. Each stream is composed of 4 residual blocks of (2, 2, 3, 6) number of layers and (1, 2, 2, 2) stride. Thus, the features after each residual block are (1x, 2x, 4x and 8x) downsampled from the input. The features from the different blocks are then concatenated at 4x dowsampling (we use average pooling to downsample further the features from the first two blocks and interpolation to upsample the features of the last block).The only different between the 2 streams is that the LiDAR one uses more features (32, 64, 128, 256) versus (16, 32, 64, 128). Finally, the features are trivially fused by concatenation along the feature dimension followed by a final residual block of 4 convolutional layers ($\text{CNN}_\text{F}$) with no downsampling, which outputs a tensor $\mathcal{F}$ with 256 features.

\paragraph{Detection Header}
The detection header is composed by two components. The first component predicts a classification score $p_{r,c}$ for each spatial location $r, c$. Each class score is predicted by a separate convolutional layer. The second component predicts the bounding box parameters $b_{r,c} = (o^x_{r,c}, o^y_{r,c}, w_{r,c}, h_{r,c}, \text{sin}\phi_{r,c}, \text{cos}\phi_{r,c})$, which are the centroid offsets from the center of the spatial cell $r, c$, width, height, sine and cosine of the heading. Finally, we perform Non-Maximum Supression (NMS) to obtain the final set of bounding boxes $\mathcal{B}$.

\paragraph{Trajectory Decoder}
Once we have the features $\mathcal{F}$ and bounding boxes $\mathcal{B}$, we apply Rotated Region of Interest Align (RRoI Align) \cite{ma2018arbitrary} to extract fixed size spatial features around each agent. We then use a 4-layer CNN with large stride ($\text{CNN}_\text{R}$) and max pooling to obtain a per-agent feature vector $\mathcal{F}_i$. \simon{Don't think we have time for this: We then update this representation using a Spatially-Aware Graph Neural Network \cite{casas2019spatially} to take into account the agent-to-agent interactions. Finally, we employ a Gated Recurrent Unit (GRU) to regress the parameters of mixture of trajectories.} More precisely, we obtain the actual parameters of the distribution as a preprocessing of the outputs of the neural network ($r_k$, $\mu_{x,k}^{(t)}$, $\mu_{y,k}^{(t)}$, $s_{l, k}^{(t)}$, $s_{c, k}^{(t)}$), as is common practice in Mixture Density Networks \cite{bishop2006pattern}: 
$$
\sigma_{l, k}^{(t)} = \exp(s_{l, k}^{(t)}); \sigma_{c, k}^{(t)} = \exp(s_{c, k}^{(t)})
$$
$$
\pi_{k} = \frac{\exp(r_{k})}{\sum_{q=1}^{K} \exp(r_{q})};
\boldsymbol{\mu}_{k}^{(t)}=\left(\begin{array}{c}{\mu_{x,k}^{(t)}} \\ {\mu_{y,k}^{(t)}}\end{array}\right)
$$
$$
\boldsymbol{b}_{k}^{(t)}=\left(\begin{array}{c}{b_{x,k}^{(t)}} \\ {b_{y,k}^{(t)}}\end{array}\right)
$$
